Lepton flavor violation in supersymmetric low-scale seesaw models

The minimal supersymmetric standard model with a low scale see-saw mechanism is presented. Within this framework, the lepton flavour violation in the charged lepton sector is thoroughly studied. Special attention is paid to the individual loop contributions due to the heavy neutrinos $N_{1,2,3}$, sneutrinos $\tilde{N}_{1,2,3}$ and soft SUSY-breaking terms. For the first time, the complete set of box diagrams is included, in addition to the photon and $Z$-boson mediated interactions. The complete set of chiral amplitudes and their associate form-factors related to the neutrinoless three-body charged lepton flavor violating decays of the muon and tau, such as $\mu \to eee$, $\tau \to \mu\mu\mu$, $\tau \to e\mu\mu$ and $\tau \to ee\mu$, as well as the coherent $\mu \to e$ conversion in nuclei, were derived. The obtained analytical results are general and can be applied to most of the New Physics models with charged lepton flavor violation. This systematic analysis has revealed the existence of two new box form factors, which have not been considered before in the existing literature in this area of physics. In the same model, the systematic study of one-loop contributions to the muon anomalous magnetic dipole moment $a_\mu$ and the electron electric dipole moment $d_e$ is performed. Special attention is paid to the effect of the sneutrino soft SUSY-breaking parameters, $B_\nu$ and $A_\nu$, and their universal CP phases ($\theta$ and $\phi$) on $a_\mu$ and $d_e$.

==> dok_kartica_hr.tex <==

\thispagestyle{empty}

\bc
{\Large \textsc{Temeljna dokumentacijska kartica}}\\
\ec

\vspace{1.0cm}

\noindent
{\large Sveu\v cili\v ste u Zagrebu \hspace{4.0cm} Doktorska disertacija\\
Prirodoslovno-matemati\v cki fakultet\\
Fizi\v cki odsjek}\\

\vspace{1.0cm}

\bc
{\Large \textbf{Nesa\cc uvanje leptonskog okusa u supersimetri\cc nim modelima
  njihalice na niskoj skali}}\\

\vspace{1.0cm}

{\large \textsc{Luka Popov}\\

\vspace{0.2cm}

Prirodoslovno-matemati\v cki fakultet, Zagreb}\\
\ec

\vspace{0.5cm}

Izlo\z en je  minimalni supersimetri\cc ni standardni model s modelom
njihalice na niskoj skali. U okviru tog modela detaljno je izu\cc eno
naru\s enje leptonskog okusa u nabijenom leptonskom sektoru. Posebna
pa\z nja posve\c ena je pojedinim doprinosima petlji koji dolaze od
te\s kih neutrina $N_{1,2,3}$, sneutrina $\widetilde{N}_{1,2,3}$ i \cc lanova
koji mekano lome supersimetriju. Po prvi put uklju\cc en je i cjelovit skup 
pravokutnih dijagrama, zajedno s fotonskim i $Z$-bozonskim interakcijama.
Izveden je cjelovit skup kiralnih amplituda i pridru\z enih im form-faktora
povezanih s tro\cc esti\cc nim CLFV raspadima miona i tau-leptona bez neutrina,
kao \s to su $\mu\to eee$, $\tau\to \mu\mu\mu$, $\tau\to \mu ee$ i 
$\tau \to ee\mu$ te $\mu\to e$ prijelazi na atomskim jezgrama. Dobiveni
analiti\cc ki rezultati su op\c eniti i mogu se primijeniti na ve\c inu
modela nove fizike koji uklju\cc uju naru\s enje nabijenog leptonskog okusa.
Ova sustavna analiza pokazala je postojanje dodatnih form-faktora koji
proizlaze iz pravokutnih dijagrama, koji u postoje\c oj literaturi iz ovog 
podru\cc ja fizike nisu bili uzimani u obzir.

U istom modelu, sustavno su izu\cc eni doprinosi na razini jedne petlje
anomalnom magnetskom dipolnom momentu miona $a_\mu$ i elektri\cc nom
dipolnom momentu elektrona $d_e$. Posebna pa\z nja posve\c ena je
u\cc inku sneutrinskih parametara koji mekano lome supersimetriju,
$B_\nu$ and $A_\nu$, kao i njihovim univerzalnim CP fazama ($\theta$ i $\phi$)
na pona\s anje $a_\mu$ i $d_e$.

\vspace{0.5cm}

\bc
(135 stranica, 169 literaturnih navoda, jezik izvornika: engleski)\\
\ec

\vspace{0.5cm}

\noindent
Klju\v cne rije\v ci: Naru\s enje leptonskog okusa, Supersimetrija,
MSSM, Mehanizam njihalice na niskoj skali, Leptonski dipolni momenti


\begin{tabular}{ll}
 & \\
Mentor: & \hskip-4ex prof.~dr.~sc.~Amon Ilakovac, Sveu\cc ili\s te u Zagrebu\\
 & \\
Ocjenjiva\cc i: 
	&  \hskip-4ex 1. prof.~dr.~sc.~Kre\s imir Kumeri\cc ki, Sveu\cc ili\s te u Zagrebu \\
	&  \hskip-4ex 2. dr.~sc.~Vuko Brigljevi\c, zn.~savj., IRB, Zagreb \\
	&  \hskip-4ex 3. prof.~dr.~sc.~Amon Ilakovac, Sveu\cc ili\s te u Zagrebu \\
	&  \hskip-4ex 4. prof.~dr.~sc.~Apostolos~Pilaftsis, Sveu\cc ili\s te~$\!$u~$\!$Manchesteru \\
	&  \hskip-4ex 5. prof.~dr.~sc.~Mirko Planini\c, Sveu\cc ili\s te u Zagrebu \\
 & \\
Zamjene:
	&  \hskip-4ex 1. prof.~dr.~sc.~Dubravko Klabu\cc ar, Sveu\cc ili\s te u Zagrebu \\
	&  \hskip-4ex 2. dr.~sc.~Kre\s o Kadija, zn.~savj., IRB, Zagreb \\
& \\
Rad prihva\c en: & 2013.
\end{tabular}


==> naslovnica_hr.tex <==

\thispagestyle{empty}

\bc

{\large \textsc{Sveu\v cili\v ste u Zagrebu}}\\
\vspace{0.2cm}
{\large \textsc{Prirodoslovno-matemati\v cki fakultet}}\\
\vspace{0.2cm}
{\large \textsc{Fizi\v cki odsjek}}\\
\vspace{2.5cm}
{\Large Luka Popov}\\

\vspace{2.8cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\huge \textbf{Nesa\cc uvanje leptonskog okusa u}}\\
\vspace{0.3cm}
{\huge \textbf{supersimetri\cc nim modelima}}\\
\vspace{0.3cm}
{\huge \textbf{njihalice na niskoj skali}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{2.7cm}

{\large Doktorska disertacija\\
predlo\v zena Fizi\v ckom odsjeku\\
Prirodoslovno-matemati\v ckog fakulteta Sveu\v cili\v sta u Zagrebu\\
radi stjecanja akademskog stupnja\\
doktora prirodnih znanosti fizike\\

\vspace{2.5cm}

Zagreb, 2013.}

\ec

\newpage
\thispagestyle{empty}
\mbox{}
